Learning Cross-lingual Visual Speech Representations

Cross-lingual self-supervised learning has been a growing research topic in the last few years. However, current works only explored the use of audio signals to create representations. In this work, we study cross-lingual self-supervised visual representation learning. We use the recently-proposed Raw Audio-Visual Speech Encoders (RAVEn) framework to pre-train an audio-visual model with unlabelled multilingual data, and then fine-tune the visual model on labelled transcriptions. Our experiments show that: (1) multi-lingual models with more data outperform monolingual ones, but, when keeping the amount of data fixed, monolingual models tend to reach better performance; (2) multi-lingual outperforms English-only pre-training; (3) using languages which are more similar yields better results; and (4) fine-tuning on unseen languages is competitive to using the target language in the pre-training set. We hope our study inspires future research on non-English-only speech representation learning.

==> tables/tab_multilingual_vs_monolingual.tex <==
\begin{table}[!t]
\small
\centering
\renewcommand\arraystretch{1.0}
\begin{tabularx}{.99\linewidth}{o  c c c c c c }
\toprule
\multirow{2}{*}{\textbf{\shortstack{Model}}} &\multicolumn{5}{c}{\textbf{Languages}}
    \\
& \textbf{en} & \textbf{it} & \textbf{pt} & \textbf{fr} & \textbf{es} & \textbf{zh} \\
\midrule
\textbf{\shortstack{Pre-Trained Data\\(Hours)}}        &1\,333        & 68          & 337         & 117         & 204         & 65 \\
\midrule
\textbf{\shortstack{Fine-Tuned Data\\(Hours)}} &30          & 40          & 73          & 72          & 62          & 60.5 \\
\midrule\midrule

\multirow{1}{*}{Monolingual} & \textbf{28.5} & 76.9 & \textbf{43.5} & \textbf{71.9} & \textbf{47.2} & \textbf{22.6} \\
\midrule
\multirow{1}{*}{Multilingual} & 32.8 & \textbf{75.7} &48.3 &73.3 &49.6 & 24.4 \\
\bottomrule
\end{tabularx}
\setlength{\belowcaptionskip}{-10pt}
\caption{\textbf{CER on monolingual and multilingual with same training hours}. We pre-train a monolingual model for each language and six multilingual models, each using the same number of pre-training hours as the monolingual model we are comparing to.}
\label{table: multilingual vs monolingual same hours}
\end{table}
